Eyes Can't Always Tell: Fusing Eye Tracking and User Priors for User Modeling under AI Advice Conditions

Modeling users' cognitive states (e.g., cognitive load and decision confidence) is essential for building adaptive AI in high-stakes decision-making. While eye tracking provides non-invasive behavioral signals correlated with cognitive effort, prior work has not systematically examined how AI assistance contexts, specifically varying advice reliability and user heterogeneity, can alter the mapping between gaze signals and cognitive states. We conducted a within-subject lab eye-tracking study (N=54) on factual verification tasks under three conditions: No-AI, Correct-AI advice, and Incorrect-AI advice. We analyze condition-dependent changes in self-reports and eye-tracking patterns and evaluate the robustness of eye-tracking-based user modeling. Results show that AI advice increases decision confidence compared to No-AI, while Correct-AI is associated with lower perceived cognitive load and more efficient gaze behavior. Crucially, predictive modeling is context-sensitive: the relationship between eye-tracking signals and cognitive states shifts across AI conditions. Finally, fusing eye-tracking features with user priors (demographics, AI literacy/experience, and propensity to trust technology) improves cross-participant generalization. These findings support condition-aware and personalized user modeling for cognitively aligned adaptive AI systems.

==> package.tex <==
% Remove the "review" option to generate the final version.
% \usepackage[review]{acl}

% Standard package includes
\usepackage{times}
\usepackage{latexsym}

% For proper rendering and hyphenation of words containing Latin characters (including in bib files)
\usepackage[T1]{fontenc}
% For Vietnamese characters
% \usepackage[T5]{fontenc}
% See https://www.latex-project.org/help/documentation/encguide.pdf for other character sets

% This assumes your files are encoded as UTF8
\usepackage[utf8]{inputenc}

% This is not strictly necessary, and may be commented out,
% but it will improve the layout of the manuscript,
% and will typically save some space.
\usepackage{microtype}

% This is also not strictly necessary, and may be commented out.
% However, it will improve the aesthetics of text in
% the typewriter font.
\usepackage{inconsolata}

% If the title and author information does not fit in the area allocated, uncomment the following
%
%\setlength\titlebox{<dim>}
%
% and set <dim> to something 5cm or larger.

% =========================================================================================

\usepackage{acronym}
\usepackage{enumitem} % Add this line


==> tables/res_gaze_tests.tex <==
\begin{table*}[!t]
\centering
\footnotesize
\setlength{\tabcolsep}{4pt} % 调整列间距
\renewcommand{\arraystretch}{0.90} % 1.2倍行距，放在\begin{tabular}之前
\begin{tabular}{@{}p{1.6cm}p{2.9cm}p{1.6cm}p{1.6cm}p{1.6cm}p{1.6cm}p{1.6cm}p{1.6cm}p{1.5cm}@{}}
\toprule
\multirow{2}{*}{\textbf{AOI}} & \multirow{2}{*}{\textbf{Comparison}} & \multicolumn{2}{c}{\textbf{Fixation}} & \multicolumn{2}{c}{\textbf{Saccade}} & \multicolumn{2}{c}{\textbf{Pupil Diameter}} & \textbf{Time To} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
& & Count & Duration & Count & Length & Overall & Fixation & \textbf{First Fix.} \\
\midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Context\\ (AOI-1)\end{tabular}} 
& No vs. Correct     & \down{.07 (.51)}  & \down{\sigtwo{.52 (.00)}} & \up{\sigtwo{2.26 (.00)}} & \up{\sigone{.26 (.01)}} & \up{.12 (.27)} & \up{.11 (.29)} & \down{\sigone{.24 (.02)}} \\ 
& No vs. Incorrect      & \down{\sigone{.22 (.04)}} & \down{\sigtwo{.63 (.00)}} & \up{\sigtwo{2.57 (.00)}} & \down{.00 (.99)} & \up{.10 (.31)} & \up{.10 (.33)} & \down{.19 (.07)} \\ 
& Correct vs. Incorrect & \down{.15 (.14)} & \down{.14 (.17)} & \down{.07 (.47)} & \down{.18 (.09)} & \up{.01 (.92)} & \down{.01 (.95)} & \down{.05 (.64)} \\ 
\midrule
\multirow{1}{*}{\begin{tabular}[c]{@{}l@{}}AI Response\end{tabular}} 
% & No vs. Correct        & \sigtwo{2.11 (.00)} & \sigtwo{2.67 (.00)} & \sigone{.23 (.03)} & \sigtwo{1.55 (.00)} & / & / & / \\ 
% & No vs. Incorrect      & \sigtwo{2.00 (.00)} & \sigtwo{2.54 (.00)} & .06 (.57) & \sigtwo{2.32 (.00)} & / & / & / \\ 
% & No vs. Correct        & -- & -- & -- & -- & -- & -- & -- \\ 
% & No vs. Incorrect      & -- & -- & -- & -- & -- & -- & -- \\ 
& Correct vs. Incorrect & \down{.12 (.24)} & \down{.16 (.13)} & \down{.15 (.15)} & \up{.00 (.97)} & \down{.03 (.74)} & \down{.03 (.78)} & \up{.01 (.89)} \\ 
\midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Rating\\ (AOI-3)\end{tabular}} 
& No vs. Correct        & \up{\sigtwo{.64 (.00)}} & \down{.05 (.66)} & \up{\sigtwo{.63 (.00)}} & \up{\sigtwo{.43 (.00)}} & \up{.11 (.29)} & \up{.12 (.24)} & \down{\sigone{.20 (.05)}} \\ 
& No vs. Incorrect      & \up{\sigtwo{.39 (.00)}} & \down{.08 (.47)} & \up{\sigtwo{.53 (.00)}} & \up{\sigtwo{.42 (.00)}} & \up{.11 (.30)} & \up{.12 (.26)} & \down{\sigtwo{.29 (.00)}} \\ 
& Correct vs. Incorrect & \down{\sigone{.23 (.03)}} & \down{.03 (.80)} & \down{.14 (.19)} & \down{.05 (.61)} & \up{.00 (.98)} & \up{.01 (.94)} & \down{.09 (.41)} \\ 
\bottomrule
\end{tabular}
% \vspace{-3.6mm}
\caption{Statistical comparisons (pairwise t-test) of eye-tracking signals across AOIs and AI conditions. Values represent effect size (p-value), p-values are color-coded: \textcolor{blue}{blue} for $p < .05$, \textcolor{red}{red} for $p < .01$; arrows indicate direction of effect (\up = first $>$ second, \down = first $<$ second); “–” denotes AOI not applicable under No-AI condition.
}
\label{tab:gaze_tests}
\vspace{-3.6mm}
\end{table*}




==> tables/stimuli_examples.tex <==
% \clearpage
% \onecolumn

\begin{table*}[!h]
\centering
\footnotesize
\renewcommand{\arraystretch}{3.0}
\begin{tabularx}{\textwidth}{>{\raggedright\arraybackslash}p{0.22\textwidth} >
{\raggedright\arraybackslash}X} 
\hline
\multicolumn{1}{l}{\textbf{Component}} & \multicolumn{1}{l}{\textbf{Content}} \\
\hline

\textbf{Factual Verification Question} & 
Is Miami a city on the American West Coast?
\\ \hline

% \textbf{AI's Answer} & 
% No, Miami is not a city on the American West Coast. 
% It's located in Florida, which is part of the southeastern region of the United States and lies along the East Coast.
% \\ \cline{1-2}

\textbf{AI's Advice\newline(Correct)} &  
% First, let’s identify where Miami is located. 
Miami is a city in the state of Florida, and it sits in the southeastern part of the United States along the Atlantic Ocean.\newline
% Now, let’s consider what is meant by the American West Coast. This term refers to the coastal states bordering the Pacific Ocean—California, Oregon, Washington, Alaska, and sometimes Hawaii. 
Since Florida is located on the East Coast, it is not part of the West Coast. Therefore, Miami is not a city on the American West Coast.
\\ \cline{1-2}

\textbf{AI's Advice\newline(Incorrect)} &  
Miami is located in the state of California, which is one of the primary West Coast states. (Here is the factual incorrectness in this step)\newline
American West Coast refers to the coastal states bordering the Pacific Ocean, California, Oregon, Washington, Alaska, and sometimes Hawaii. 
% Despite that, when we review the actual location of Miami, it's evident that it’s not on the Pacific Ocean but on the Atlantic, which confirms it’s not a city on the West Coast.\newline
So Miami is on the American West Coast.
\\ \hline
\end{tabularx}
\caption{An example factual verification question and the AI advice shown to participants: the advice is either correct or incorrect, depending on the condition.}
\vspace{-6.6mm}
\end{table*}
